J-PLUS: Turning Off the Bright Stars

Photometric surveys require precise point spread function (PSF) characterization, as it varies across filters and is crucial for accurate photometry and low surface brightness (LSB) studies. However, the small PSF size provided by default pipelines suits only barely resolved objects, making it difficult to analyze regions near bright stars (rendering those regions unusable). These components are then combined to generate a final PSF for each exposure and filter, spanning 15 mag arcsec-2 in surface brightness and 4 arcmin in radius in the broad bands. In narrow-band filters, the J-PLUS PSF exhibits two rings, whereas in broad-band filters, only one ring is observed. Additionally, the position of the ring shifts with filter wavelength: as the filters become redder, the ring radius increases. We find that there is no significant variation in the extended PSF observed as a function of time (within 2.5h) or position in the field of view. The radial profile of NGC 4212 (which is close to a star) is also studied before/after PSF-subtraction. We developed a novel method to determine the central coordinates of saturated stars, and classify stars without using Gaia magnitudes. Additionally, mirror reflections are automatically detected and masked. Furthermore, in combining different stars and various components of the PSF, we avoided the use of a fixed radius by introducing a new method that does not depend on radial measurements. Accurate characterization of the extended PSF and its subtraction improves sky subtraction, increases the effective area of the survey by about 10%, and enables the study of extended large LSB features in wide area surveys like J-PLUS. Our pipeline is published as free software (GNU GPLv3) an can be customized to other surveys such as J-PAS, where its impact will be even greater due to its depth. This paper is fully reproducible and produced from Commit 4860c70.

==> project <==
#!/bin/sh
#
# High-level script to manage the project.
# Run './project --help' for a description of how to use it.
#
# Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
# Copyright (C) 2021-2025 Raul Infante-Sainz <infantesainz@gmail.com>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.


# Basic settings
# --------------
# Stop the script if there are any errors.
set -e





# Default option values
jobs=0     # 0 is for the default for the 'configure.sh' script.
group=
debug=
quiet=0
timing=0
host_cc=0
offline=
operation=
build_dir=
input_dir=
keep_going=
check_config=
make_targets=
software_dir=
pauseformsg=1
clean_texdir=0
prepare_redo=0
highlightnew=0
all_highlevel=0
existing_conf=0
highlightnotes=0
scriptname="./project"





# Parse the options
# -----------------
#
# Separate command-line arguments from options. Then put the option value
# into the respective variable.
#
# Each option has two lines because we want to process both these formats:
# '--name=value' and '--name value'. The former (with '=') is a single
# command-line argument, so we just need to shift the counter by one. The
# latter (without '=') is two arguments, so we'll need two shifts.
#
# Note on the case strings: for every option, we need three lines: one when
# the option name and value are separate. Another when there is an equal
# between them, and finally one where the value is immediately after the
# short-format. This exact order is important. Otherwise, there will be a
# conflict between them.

print_help() {
    # Print the output.
    cat <<EOF
Usage: $scriptname configure [OPTIONS]
       $scriptname shell     [OPTIONS]
       $scriptname make      [OPTIONS]

Top-level script to manage the reproducible project. The high-level
operation is defined by the (mandatory) second argument:

  configure    - Configure project for this machine (e.g., build software).
  make         - Run the project (do analysis and build outputs).
  shell        - Execute the project's shell for interactive testing.

RECOMMENDATION: If this is the first time you are configuring this
template, please don't use the options and let the script explain each
parameter in full detail by simply running './project configure'.

Project 'make' special tagets
  ./project make           Build the project on one thread
  ./project make -jN       Built the project in parallel on N threads.
  ./project make clean     Clean all files generated by 'make' (not software).
  ./project make texclean  Clean all files built by (La)TeX.
  ./project make distclean Clean everything (including compiled software).
  ./project make dist      Produce a LaTeX-ready-to-build distribution tarball
                           ('tar.gz') of the project. This is ready to be
                           uploaded to servers like 'arXiv.org'.
  ./project make dist-lzip Similar to 'dist', but compress to '.tar.lz'.
  ./project make dist-zip  Similar to 'dist', but compress to '.zip'.
  ./project make dist-software  Build a .tar.gz tarball containing all
                                software source tarballs necessary for the
                                project.

With the options below you can modify the default behavior.
Configure options:
      --all-highlevel      Build all high-level software (for development).
  -b, --build-dir=STR      Top directory to build the project in.
      --check-config       During configuration, show what is being built.
      --clean-texdir       Remove possibly existing build-time subdirectories
                           under the project's 'tex/' directory (can happen
                           when source is from arXiv for example).
  -e, --existing-conf      Use (possibly existing) local configuration.
  -i, --input-dir=STR      Directory containing input datasets (optional).
      --host-cc            Use host system's C compiler, don't build GCC.
      --quiet              Do not print basic info messages (with '-e').
      --no-pause           Do not sleep/pause after basic info messages.
  -s, --software-dir=STR   Directory containing necessary software tarballs.

Configure and Make options:
  -d, --debug[=FLAGS]      In configure: use -j1, no -k, and no Zenodo check.
                           In make: 'FLAGS' will be directly passed to 'make'.
  -k, --keep-going         Keep going when some targets can't be made.
  -g, --group=STR          Build and run with write permissions for a group.
  -j, --jobs=INT           Number of threads to build/run the software.
  -?, --help               Print this help list.

Make (analysis) options:
  -p, --prepare-redo       Re-do preparation (only done automatically once).
  -t, --timing             Starting and ending times written in 'timing.txt'.

Make (final PDF) options:
      --refresh-bib        Force refresh the bibliography.
      --highlight-all      Activate '--highlight-new' & '--highlight-notes'.
      --highlight-new      Highlight '\new' parts of text as green.
      --highlight-notes    Show '\tonote' regions as red text in PDF.

Mandatory or optional arguments to long options are also mandatory or optional
for any corresponding short options.

Maneage URL: https://maneage.org

Report bugs to mohammad@akhlaghi.org
EOF
}

on_off_option_error() {
    if [ "x$2" = x ]; then
        echo "$scriptname: '$1' doesn't take any values."
    else
        echo "$scriptname: '$1' (or '$2') doesn't take any values."
    fi
    exit 1
}

check_v() {
    if [ x"$2" = x ]; then
        echo "$scriptname: option '$1' requires an argument."
        echo "Try '$scriptname --help' for more information."
        exit 1;
    fi
}

func_operation_set() {
    if [ x$operation = x ]; then
        operation=$1
    else
        echo "Only one operation ('configure', 'make' or 'shell') may be given."
        exit 1
    fi
}

while [ $# -gt 0 ]
do
 case $1 in
  # Main operation.
  configure)    func_operation_set $1; shift;;
  make)         func_operation_set $1; shift;;
  shell)        func_operation_set $1; shift;;

  # Configure options:
  -e|--existing-conf)    existing_conf=1;                                                          shift;;
  -e*|--existing-conf=*) on_off_option_error --existing-conf -e;;
  --host-cc)             host_cc=1;                                                                shift;;
  --host-cc=*)           on_off_option_error --host-cc;;
  --offline)             offline=1;                                                                shift;;
  --offline=*)           on_off_option_error --offline;;
  -i|--input-dir)        input_dir="$2";                             check_v "$1" "$input_dir";    shift;shift;;
  -i=*|--input-dir=*)    input_dir="${1#*=}";                        check_v "$1" "$input_dir";    shift;;
  -i*)                   input_dir=$(echo    "$1" | sed -e's/-i//'); check_v "$1" "$input_dir";    shift;;
  -s|--software-dir)     software_dir="$2";                          check_v "$1" "$software_dir"; shift;shift;;
  -s=*|--software-dir=*) software_dir="${1#*=}";                     check_v "$1" "$software_dir"; shift;;
  -s*)                   software_dir=$(echo "$1" | sed -e's/-s//'); check_v "$1" "$software_dir"; shift;;
  --check-config)        check_config=1;                                                           shift;;
  --check-config=*)      on_off_option_error --check-config;;
  --clean-texdir)        clean_texdir=1;                                                           shift;;
  --clean-texdir=*)      on_off_option_error --clean-texdir;;
  --all-highlevel)       all_highlevel=1;                                                          shift;;
  --all-highlevel=*)     on_off_option_error --all-highlevel;;
  --no-pause)            pauseformsg=0;                                                            shift;;
  --no-pause=*)          on_off_option_error --no-pause;;
  --quiet)               quiet=1;                                                                  shift;;
  --quiet=*)             on_off_option_error --quiet;;

  # Configure and Make options:
  -b|--build-dir)        build_dir="$2";                             check_v "$1" "$build_dir";shift;shift;;
  -b=*|--build-dir=*)    build_dir="${1#*=}";                        check_v "$1" "$build_dir";shift;;
  -b*)                   build_dir=$(echo    "$1" | sed -e's/-b//'); check_v "$1" "$build_dir";shift;;
  -g|--group)            group="$2";                                 check_v group "$group";   shift;shift;;
  -g=*|--group=*)        group="${1#*=}";                            check_v group "$group";   shift;;
  -g*)                   group=$(echo   "$1" | sed -e's/-g//');      check_v group "$group";   shift;;
  -j|--jobs)             jobs="$2";                                  check_v jobs  "$jobs";    shift;shift;;
  -j=*|--jobs=*)         jobs="${1#*=}";                             check_v jobs  "$jobs";    shift;;
  -j*)                   jobs=$(echo "$1" | sed -e's/-j//');         check_v jobs  "$jobs";    shift;;
  -k|--keep-going)       keep_going="--keep-going";                                            shift;;
  -k=*|--keep-going=*)   on_off_option_error --keep-going -k;;
  -k*)                   on_off_option_error --keep-going -k;;
  -'?'|--help)           print_help; exit 0;;
  -'?'*|--help=*)        on_off_option_error --help -?;;

  # Make options (analysis):
  -p|--prepare-redo)     prepare_redo=1;                                                  shift;;
  -p=*|--prepare-redo=*) on_off_option_error --prepare-redo;                              shift;;
  -t|--timing)           timing=1;                                                        shift;;
  -t=*|--timing=*)       on_off_option_error --timing;                                    shift;;

  # Make options (final PDF):
  --refresh-bib)         [ -f tex/src/references.tex ] && touch tex/src/references.tex;   shift;;
  --highlight-all)       highlightnew=1; highlightnotes=1;                                shift;;
  --highlight-all=*)     on_off_option_error --highlight-new;;
  --highlight-new)       highlightnew=1;                                                  shift;;
  --highlight-new=*)     on_off_option_error --highlight-new;;
  --highlight-notes)     highlightnotes=1;                                                shift;;
  --highlight-notes=*)   on_off_option_error --highlight-notes;;
  -d|--debug)            if [ x$operation = x ]; then
                             echo "Please set the operation before calling '--debug'"; exit 1
                         elif [ x$operation = xconfigure ]; then debug=a;   shift;
                         elif [ x$operation = xmake ]; then
                             if [ x"$2" = x ]; then
                                 echo "In make-mode, '--debug' needs a value; see GNU Make manual"; exit 1
                             else debug="$2"; check_v debug "$debug"; shift;shift; fi
                         else
                             echo "Operation '$operation' not recognized, please use 'configure' or 'make'"
                         fi;;
  -d=*|--debug=*)        debug="${1#*=}";                       check_v debug "$debug";   shift;;
  -d*)                   debug=$(echo "$1" | sed -e's/-d//');   check_v debug "$debug";   shift;;

  # Unrecognized option:
  -*) echo "$scriptname: unknown option '$1'"; exit 1;;

  # Not an option, an argument (so its a Make target).
  *) make_targets="$make_targets $1"; shift;;
 esac
done





# Check configuration status
# --------------------------
if ! [ x$check_config = x ]; then
    # Find the color option to pass to 'ls'. Note that '--color' (for GNU
    # Coreutils 'ls') should be checked first because it also has '-G', but
    # for something else.
    if   ls --color 2> /dev/null > /dev/null; then coloropt="--color=auto"
    elif ls -G      2> /dev/null > /dev/null; then coloropt="-G"
    else                               coloropt=""
    fi

    # Print a notice to let the user know what is happening.
    cat <<EOF

This is an infinite loop that will print what software are being built at
every moment. It is actually a listing ('ls' command) of the temporary
directory where software source code are unpacked while they are being
built. If the project isn't being configured, the output (every second)
will either be empty (only a date) or a with an error about a non-existant
directory. This feature is thus only useful when the project's software are
being built.

EOF

    # Run the infinite loop. To be able to find the last built programs, we
    # need to put all the Python programs and high-level program into one
    # directory.
    checkdir=.local/version-info/.for-check-config
    while true; do

        # Make sure the '.build' directory has already been created.
        echo;
        echo "========================"
        if [ -d .build ]; then
            echo "$(date)    [[press CTRL-C to stop]]";
            echo "--- Currently being built:"
            if [ -d .build/software/build-tmp ]; then
                ls $coloropt .build/software/build-tmp || junk=1;
            fi

            # Make the temporary directory, delete its contents, then put
            # new links of all built software.
            if ! [ -d $checkdir ]; then mkdir $checkdir; fi
            rm -f $checkdir/*

            # Check if any programs exist in the given directory yet.
            printresults=0
            check=$(ls .local/version-info/python/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/python/*  $checkdir/
            fi
            check=$(ls .local/version-info/proglib/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/proglib/* $checkdir/
            fi

            # If something was actually found, then print them.
            if [ $printresults = 1 ]; then
                echo "--- Last 5 packages that were built:"

                # Then sort all the links based on the most recent dates of
                # the files they link to (with '-L').
                ls -Llt $checkdir  \
                    | awk '/^-/ && c++<5 {printf "[at %s] %s\n", \
                                                 $(NF-1), $NF}'
            fi
        else
            cat <<EOF
The connection to the build directory (.build) is not yet created.

If you have just ran './project configure', it should be created and will
be used in a few seconds to report the build status of various software.
If not, please run './project configure' (in another terminal) and you will
see the results shortly afterwards.
EOF
        fi
        echo "========================"

        # Wait for the next round of checks.
        sleep 1
    done
    exit 0
fi





# Group check
# -----------
if ! [ x$group = x ]; then

    # Check if group is usable.
    if ! sg "$group" "echo Group \'$group\' exists"; then
        printf "$scriptname: '$group' is not a usable group name on "
        printf "this system. TIP: you can use the 'groups' command "
        printf "to see your groups)\n"
        exit 1
    fi

    # Set the group option for running Make.
    gopt="maneage_group_name=$group"
fi





# Build directory symbolic links
# ------------------------------
#
# The source directory will contain two symbolic links that point to the
# build directory:

#   - .build: the top build directory.
#
#   - .local: the second to the top software installed directory. They are
#     used during the configuration phase to simplify commands and are also
#     very useful during the development of a maneage'd project (to easily
#     get to the build directory or execut Maneage'd software).
#
# This needs to be done on every run because:
#   - './project configure' can be run with a new build directory, and
#     keeping the old '.build' conflicts with the new build directory
#     that the user gave.
#   - './project make' or './project shell' (within a newly cloned source
#     directory from inside a container): the links do not exist but have
#     to be set to the container's build directory.
#   - This is not an expensive operation.
if ! [ x"$build_dir" = x ]; then
    rm -f .build .local
    ln -s $build_dir .build
    ln -s $build_dir/software/installed .local
fi





# Function to validate configuration
# ----------------------------------
#
# Check if the configuration is missing/incomplete
configuration_check() {
    confdone=software/config/hardware-parameters.tex
    if ! [ -f .build/$confdone ]; then
        cat <<EOF

The project is either (1) not configured on this system, or (2) the
configuration wasn't successful.

(1) If it hasn't been configured at all, use the command below to configure
it (set a build directory and let it build its necessary software in it).

      $ ./project configure

(2) If it has been configured, but the configuration failed in a step, you
can re-configure it using your previous settings with the command
below. All successful steps will be skipped, allowing a fast completion.

      $ ./project configure -e

If there was a problem, please let us know by filling this online form:
      http://savannah.nongnu.org/support/?func=additem&group=reproduce

EOF
        exit 1
    fi
}





# Function for TeX Preparations
# -----------------------------
#
# Make sure that the necessary analysis directories directory exist in the
# build directory. These will be necessary in various phases of hte
# analysis and having them inside the lower-level Make steps will require
# setting them as prerequisites for many basic jobs (thus making the
# Makefiles harder to read and add potentials for bugs: forgetting to add
# them for example). Also, we don't want the configure phase to make any
# edits in the analysis directory, so they are not built there.
tex_preparations () {

    # Extract the location of the build directory.
    bdir=$(.local/bin/realpath .build)

    # We are using our custom-built 'mkdir' which is guaranteed to have the
    # '-p' option (that will also build intermediate directories) and won't
    # complain if the directory already exists.
    badir=$bdir/analysis
    texdir=$badir/tex
    btexdir=$texdir/build
    tikzdir=$btexdir/tikz
    mtexdir=$texdir/macros
    .local/bin/mkdir -p $mtexdir $btexdir $tikzdir

    # If 'tex/build' and 'tex/tikz' are symbolic links then 'rm -f'
    # will delete them and we can continue. However, when the project
    # is being built from the tarball (from arXiv for example), these
    # two are not symbolic links but actual directories with the
    # necessary built-components to build the PDF in them. In this
    # case, because 'tex/build' is a directory, 'rm -f' will fail, so
    # we'll just rename the two directories (as backup) and let the
    # project build the proper symbolic links afterwards.
    if rm -f tex/build; then
        rm -f tex/tikz
    else
        mv tex/tikz  tex/tikz-from-tarball
        mv tex/build tex/build-from-tarball
    fi

    # Build the symbolic links.
    if ! [ -L tex/tikz ]; then ln -s "$tikzdir" tex/tikz; fi
    if ! [ -L tex/build ]; then ln -s "$texdir" tex/build; fi
}





# Function to run in controlled environment
# -----------------------------------------
#
# Controlling the environment is necessary for running the analysis. Like
# the other funcitons here, this is defined to simplify the high-level code
# within the 'make)' switch statement.
perms="u+r,u+w,g+r,g+w,o-r,o-w,o-x"
controlled_env() {

    # Get the full address of the build directory:
    bdir=`.local/bin/realpath .build`

    # Remove all existing environment variables (with 'env -i') and only
    # use some pre-defined environment variables, then build the project.
    envmake=".local/bin/env -i HOME=$bdir sys_rm=$(which rm) $gopt"
    envmake="$envmake highlightnew=$highlightnew"
    envmake="$envmake highlightnotes=$highlightnotes .local/bin/make"
    envmake="$envmake --no-builtin-rules --no-builtin-variables -f $1"
    envmake="$envmake $keep_going"
    if ! [ x"$debug" = x  ]; then envmake="$envmake --debug=$debug"; fi

    # Set the number of jobs. Note that for the 'configure.sh' script the
    # default value has to be 0, so the default is the maximum number of
    # threads. But here, the default value is 1.
    if ! [ x"$jobs"  = x0 ]; then envmake="$envmake -j$jobs";  fi

    # Run the project
    if [ x"$group" = x ]; then
        $envmake $make_targets
    else
        # Set the group and permission flags.
        sg "$group" "umask $perms && $envmake $make_targets"
    fi
}





# Do requested operation
# ----------------------
configscript=./reproduce/software/shell/configure.sh
case $operation in

    # Build the project's software.
    configure)

        # Set executable flags
        # --------------------
        #
        # In some scenarios (for example when using a tarball from arXiv),
        # it may happen that the host server has removed the executable
        # flags of all the files. In 'README.md' we instruct the readers on
        # setting the executable flag of this script. But we don't want the
        # user to have to worry about any other file that needs an
        # executable flag.
        #
        # Basically, all the project shell scripts need executable flags so
        # to make sure they have them, we are activating the executable
        # flags by default here every time './project configure' is run. If
        # any other file in your project needs such flags, add them here.
        if ! [ -x reproduce/software/shell/configure.sh ]; then
            chmod +x reproduce/analysis/bash/* \
                     reproduce/software/shell/* \
                     reproduce/software/config/*.sh
        fi

        # If the user requested, clean the TeX directory from the extra
        # (to-be-built) directories that may already be there (and will not
        # allow the configuration to complete).
        if [ x"$clean_texdir" = x1 ]; then
            rm -rf tex/build tex/tikz
        fi

        # Variables to pass to the configuration script.
        export jobs=$jobs
        export debug=$debug
        export quiet=$quiet
        export host_cc=$host_cc
        export offline=$offline
        export build_dir=$build_dir
        export input_dir=$input_dir
        export scriptname=$scriptname
        export pauseformsg=$pauseformsg
        export maneage_group_name=$group
        export software_dir=$software_dir
        export existing_conf=$existing_conf
        export all_highlevel=$all_highlevel

        # Run the configuration script
        if [ x"$group" = x ]; then
            $configscript
        else
            # Set the group and permission flags.
            sg "$group" "umask $perms && $configscript"

            # Set the group writing permission for everything in the
            # installed software directory. The common build process sets
            # the writing permissions of the installed programs/libraries
            # to '755'. So group members can't write over a file. This
            # creates problems when another group member wants to update
            # the software for example. We thus need to manually add the
            # group writing flag to all installed software files.
            printf "Enabling group writing permission on all installed "
            printf "software...\n"
            .local/bin/chmod -R g+w .local/;
        fi
        ;;





    # Batch execution of the project.
    make)

        # Make sure the configure script is complete and necessary LaTeX
        # directories are in place.
        configuration_check
        tex_preparations

        # Register the start of this run if requested (we are appending the
        # new information so previous information is preserved until the
        # user intentionally deletes/cleans it).
        if [ $timing = 1 ]; then echo "start: $(date)" >> timing.txt; fi

        # Add a extra preparation step for defining J-PLUS inputs.
        if ! [ -f .build/analysis/pre-preparation-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-pre-prepare.mk
        fi

        # Run data preparation phase (optionally build Makefiles with
        # special values for optimizing the main 'top-make.mk'). But note
        # that data preparation is only done automatically the first time
        # the project is built (when '.build/analysis/preparation-done.mk'
        # doesn't yet exist). After that, if the user wants to re-do the
        # preparation they have to use the '--prepare-redo' option.
        if ! [ -f .build/analysis/preparation-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-prepare.mk
        fi

        # Call top-make (highest level analysis Makefile).
        controlled_env reproduce/analysis/make/top-make.mk

        # Register the time of the project's ending.
        if [ $timing = 1 ]; then echo "end:   $(date)" >> timing.txt; fi
        ;;





    # Interactive shell of Maneage.
    shell)

        # Make sure the configure script has been completed properly.
        configuration_check

        # Run the project's own shell without inheriting any environment
        # from the host. The 'TERM' environment variable is necessary for
        # tools like some text editors.
        bdir=$(.local/bin/realpath .build)
        instdir="$bdir"/software/installed
        bindir="$bdir"/software/installed/bin
        rcfile=$(pwd)/reproduce/software/shell/bashrc.sh
        .local/bin/env -i \
            HOME="$bdir" \
            TERM="$TERM" \
            PATH="$bindir" \
            CCACHE_DISABLE=1 \
            PROJECT_STATUS=shell \
            SHELL="$bindir"/bash \
            COLORTERM="$COLORTERM" \
            PROJECT_RCFILE="$rcfile" \
            LDFLAGS=-L"$instdir"/lib \
            CPPFLAGS=-I"$instdir"/include \
            LD_LIBRARY_PATH="$instdir"/lib \
            OMPI_MCA_plm_rsh_agent=/bin/false \
            PYTHONPATH="$instdir"/lib/python/site-packages \
            PYTHONPATH3="$instdir"/lib/python/site-packages \
            PS1="[\[\033[01;35m\]maneage@\h \W\[\033[32m\]\[\033[00m\]]$ " \
            "$bindir"/bash --noprofile --rcfile "$rcfile"
        ;;





    # Operation not specified.
    *)
        cat <<EOF

No operation defined!

Please run with '--help' for more information.
(TIP: available operations are: 'configure', 'make', or 'shell').

EOF
        exit 1
        ;;
esac


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
       author = {{Lang}, Dustin and {Hogg}, David W. and {Mierle}, Keir and {Blanton}, Michael and {Roweis}, Sam},
        title = "{Astrometry.net: Blind Astrometric Calibration of Arbitrary Astronomical Images}",
      journal = {AJ},
     keywords = {astrometry, catalogs, instrumentation: miscellaneous, methods: data analysis, methods: statistical, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {139},
       number = {5},
        pages = {1782-1800},
          doi = {10.1088/0004-6256/139/5/1782},
archivePrefix = {arXiv},
       eprint = {0910.2233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139.1782L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {JOSS},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
       author = {{Behnel}, Stefan and {Bradshaw}, Robert and {Citro}, Craig and {Dalcin}, Lisandro and {Seljebotn}, Dag Sverre and {Smith}, Kurt},
        title = "{Cython: The Best of Both Worlds}",
      journal = {Computing in Science and Engineering},
         year = 2011,
        month = mar,
       volume = {13},
       number = {2},
        pages = {31-39},
          doi = {10.1109/MCSE.2010.118},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216-231},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astron.Comput.},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {759-771},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
       author = {{Erwin}, Peter},
        title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
      journal = {ApJ},
     keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {226},
        pages = {226},
          doi = {10.1088/0004-637X/799/2/226},
archivePrefix = {arXiv},
       eprint = {1408.1097},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/kiwisolver.tex <==
%% Copyright (C) 2025-2025 Boud Roukema <boud@cosmo.torun.pl>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cassowary2001,
   author = {{Grudin}, Jonathan and {Badros}, Greg J. and {Borning}, Alan and {Stuckey}, Peter J.},
    title = "{The Cassowary linear arithmetic constraint solving algorithm}",
    journal = {ACM Transactions on Computer-Human Interaction},
       year = 2001,
      month = dec,
     volume = {8},
     number = {4},
      pages = {267-306},
        doi = {10.1145/504704.504705},
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{matplotlib2007,
       author = {{Hunter}, John D.},
        title = "{Matplotlib: A 2D Graphics Environment}",
      journal = {CiSE},
     keywords = {Python, Scripting languages, Application development, Scientific programming},
         year = 2007,
        month = may,
       volume = {9},
       number = {3},
        pages = {90-95},
          doi = {10.1109/MCSE.2007.55},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007CSE.....9...90H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/missfits.tex <==
%% Copyright (C) 2020-2025 Surena Fatemi <surena.fatemi@ipm.ir>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{missfits,
       author = {{Marmo}, C. and {Bertin}, E.},
        title = "{MissFITS and WeightWatcher: Two Optimised Tools for Managing FITS Data.}",
      journal = {ASPC},
         year = 2008,
       volume = {394},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {619},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ASPC..394..619M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
       author = {{Dalcin}, Lisandro D. and {Paz}, Rodrigo R. and {Kler}, Pablo A. and {Cosimo}, Alejandro},
        title = "{Parallel distributed computing using Python}",
      journal = {Advances in Water Resources},
         year = 2011,
        month = sep,
       volume = {34},
       number = {9},
        pages = {1124-1139},
          doi = {10.1016/j.advwatres.2011.04.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2020,
       author = {{Harris}, Charles R. and {Millman}, K. Jarrod and {van der Walt}, St{\'e}fan J. and {Gommers}, Ralf and {Virtanen}, Pauli and {Cournapeau}, David and {Wieser}, Eric and {Taylor}, Julian and {Berg}, Sebastian and {Smith}, Nathaniel J. and {Kern}, Robert and {Picus}, Matti and {Hoyer}, Stephan and {van Kerkwijk}, Marten H. and {Brett}, Matthew and {Haldane}, Allan and {del R{\'\i}o}, Jaime Fern{\'a}ndez and {Wiebe}, Mark and {Peterson}, Pearu and {G{\'e}rard-Marchant}, Pierre and {Sheppard}, Kevin and {Reddy}, Tyler and {Weckesser}, Warren and {Abbasi}, Hameer and {Gohlke}, Christoph and {Oliphant}, Travis E.},
        title = "{Array programming with NumPy}",
      journal = {Nature},
     keywords = {Computer Science - Mathematical Software, Statistics - Computation},
         year = 2020,
        month = sep,
       volume = {585},
       number = {7825},
        pages = {357-362},
          doi = {10.1038/s41586-020-2649-2},
archivePrefix = {arXiv},
       eprint = {2006.10256},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.585..357H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/r-cran.tex <==
%% Copyright (C) 2022-2025 Boud Roukema <boud@cosmo.torun.pl>
%% Copyright (C) 2022-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{RIhakaGentleman1996,
      author = {{Ihaka}, Ross and {Gentleman}, Robert},
       title = "{R: A language for data analysis and graphics}",
     journal = {J.Comput.Graph.Stat.},
        year = {1996},
      volume = {5},
      number = {3},
       pages = {299-314},
         DOI = {10.1080/10618600.1996.10474713},
        ISSN = {10618600},
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2020,
       author = {{Virtanen}, Pauli and {Gommers}, Ralf and {Oliphant}, Travis E. and {Haberland}, Matt and {Reddy}, Tyler and {Cournapeau}, David and {Burovski}, Evgeni and {Peterson}, Pearu and {Weckesser}, Warren and {Bright}, Jonathan and {van der Walt}, St{\'e}fan J. and {Brett}, Matthew and {Wilson}, Joshua and {Millman}, K. Jarrod and {Mayorov}, Nikolay and {Nelson}, Andrew R.~J. and {Jones}, Eric and {Kern}, Robert and {Larson}, Eric and {Carey}, C.~J. and {Polat}, {\.I}lhan and {Feng}, Yu and {Moore}, Eric W. and {VanderPlas}, Jake and {Laxalde}, Denis and {Perktold}, Josef and {Cimrman}, Robert and {Henriksen}, Ian and {Quintero}, E.~A. and {Harris}, Charles R. and {Archibald}, Anne M. and {Ribeiro}, Ant{\^o}nio H. and {Pedregosa}, Fabian and {van Mulbregt}, Paul and {SciPy 1. 0 Contributors}},
        title = "{SciPy 1.0: fundamental algorithms for scientific computing in Python}",
      journal = {Nature Methods},
     keywords = {Computer Science - Mathematical Software, Computer Science - Data Structures and Algorithms, Computer Science - Software Engineering, Physics - Computational Physics},
         year = 2020,
        month = feb,
       volume = {17},
        pages = {261-272},
          doi = {10.1038/s41592-019-0686-2},
archivePrefix = {arXiv},
       eprint = {1907.10121},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatMe..17..261V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {1-28},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}


==> reproduce/software/shell/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the 'MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/shell/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the 'MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> tex/build/macros/dependencies-bib.tex <==


@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> tex/src/fig-psf-effect-color.tex <==
%% Insert the images.
\begin{tikzpicture}


  %% Insert images
  \node[anchor=north, line width=0.5mm,
        inner sep=0.2\pgflinewidth] (img) at (-0.1\linewidth,0.2\linewidth)
       {\includegraphics [width=1.1\linewidth]
        {tex/build/figures/psf-detection/color-g-r.pdf}};

\end{tikzpicture}


==> tex/src/preamble-biblatex.tex <==
%% Biblatex settings.
%%
%% Settings necessary to make the bibliography with Biblatex. Keeping all
%% BibLaTeX settings in a separate preamble was done in the spirit of
%% modularity to 1) easily managable, 2) If a similar BibLaTeX
%% configuration is necessary in another LaTeX compilation, this file can
%% just be copied there and used.
%%
%% USAGE:
%%  - 'tex/src/references.tex': the file containing Bibtex source of each
%%     reference. The file suffix doesn't have to be '.bib'. This naming
%%     helps in clearly identifying the files and avoiding places that
%%     complain about '.bib' files.
%
%% Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%% Copyright (C) 2022-2025 Sepideh Eskandarlou <sepideh.eskandarlou@gmail.com>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.




%% To break up highlighted text (for example texttt when some it is on the
%% line break) and also to no underline emphasized words (like journal
%% titles in the references).
\usepackage[normalem]{ulem}





%% For quotation signs (sometimes used by BibLaTeX)
\usepackage{csquotes}





%% To define colors
\usepackage{xcolor}





% Basic BibLaTeX settings
\usepackage[
    doi=false,
    url=false,
    dashed=false,
    eprint=false,
    maxbibnames=2,
    minbibnames=1,
    hyperref=true,
    maxcitenames=2,
    mincitenames=1,
    giveninits=true,
    style=authoryear,
    uniquelist=false,
    backend=biber,natbib]{biblatex}
\DeclareFieldFormat[article]{pages}{#1}
\DeclareFieldFormat{pages}{\mkfirstpage[{\mkpageprefix[bookpagination]}]{#1}}
\addbibresource{tex/src/references.tex}
\addbibresource{tex/build/macros/dependencies-bib.tex}
\renewbibmacro{in:}{}
\AtEveryBibitem{\clearfield{month}}
\renewcommand*{\bibfont}{\footnotesize}
\DefineBibliographyStrings{english}{references = {References}}

%% Include the adsurl field key into those that are recognized:
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map{
      \step[fieldsource=adsurl,fieldtarget=iswc]
      \step[fieldsource=gbkurl,fieldtarget=iswc]
    }
  }
}

%% Set the color of the doi link to mymg (magenta) and the ads links
%% to mypurp (or purple):
\definecolor{mypurp}{cmyk}{0.75,1,0,0}
\newcommand{\doihref}[2]{\href{#1}{\color{magenta}{#2}}}
\newcommand{\adshref}[2]{\href{#1}{\color{mypurp}{#2}}}
\newcommand{\blackhref}[2]{\href{#1}{\color{black}{#2}}}

%% Define a format for the printtext commands in
%% DeclareBibliographyDriver to make links for the doi, ads link and
%% arxiv link:
\DeclareFieldFormat{doilink}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{adslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}
\DeclareFieldFormat{arxivlink}{
  \iffieldundef{eprint}{#1}{\href{http://arxiv.org/abs/\thefield{eprint}}{#1}}}

\DeclareListFormat{doiforbook}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{googlebookslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}

%% Set the formatting to make the last three values into the
%% appropriate link. Note that the % signs are necessary. Without
%% them, the items will be indented.
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \ifdefined\makethesis\printtext{\usebibmacro{title}}\fi%
  \newunit%
  \printtext[doilink]{\usebibmacro{journal}}%
  \addcomma%
  \printtext[adslink]{\printfield{volume}}%
  \addcomma%
  \printtext[arxivlink]{\printfield{pages}}%
  \addperiod%
}

\DeclareBibliographyDriver{book}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \printtext{\usebibmacro{title}}%
  \addperiod%
  \addspace%
  \printlist[doiforbook]{publisher}%
  \addcomma%
  \addspace%
  \printfield[googlebookslink]{edition}%
  \printtext{ ed.}%
  \addperiod%
}

%% In order to have et al. instead of et al.,:
\renewcommand*{\nameyeardelim}{\addspace}


==> tex/src/preamble-maneage-default-style.tex <==
%% General paper's style settings.
%
%% This preamble can be completely ignored when including this TeX file in
%% another style. This is done because this LaTeX build is meant to be an
%% initial/internal phase or part of a larger effort, so it has a basic
%% style defined here as a preamble. To ignore it, uncomment or delete the
%% respective line in 'paper.tex'.
%
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.





%% Font.
\usepackage[T1]{fontenc}
\usepackage{newtxtext}
\usepackage{newtxmath}





%% Print size
\usepackage[a4paper, includeheadfoot, body={18.7cm, 24.5cm}]{geometry}





%% Set the distance between the columns if two columns:
\setlength{\columnsep}{0.75cm}





% To allow figures to take up more space on the top of the page:
\renewcommand{\topfraction}{.99}
\renewcommand{\bottomfraction}{.7}
\renewcommand{\textfraction}{.05}
\renewcommand{\floatpagefraction}{.99}
\renewcommand{\dbltopfraction}{.99}
\renewcommand{\dblfloatpagefraction}{.99}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{0}
\setcounter{totalnumber}{2}
\setcounter{dbltopnumber}{1}





%% To make the footnotes align:
\usepackage[hang]{footmisc}
\setlength\footnotemargin{10pt}





%For including time in the title:
\usepackage{datetime}





%% Define the abstract environment
\renewenvironment{abstract}
 {\vspace{-0.5cm}\small%
  \list{}{%
    \setlength{\leftmargin}{2cm}%
    \setlength{\rightmargin}{\leftmargin}%
  }%
  \item\relax}
 {\endlist}





%% To keep the main page's code clean.
\newcommand{\includeabstract}[1]{%
\twocolumn[%
  \begin{@twocolumnfalse}%
    \maketitle%
    \begin{abstract}%
    #1%
    \end{abstract}%
    \vspace{1cm}%
  \end{@twocolumnfalse}%
  ]%
}





%% Basic header style
%% ------------------
%
%% The steps below are to use the necessary LaTeX packages to get the demo
%% Maneage paper running with a reasonably looking, custom paper style. If
%% you are using a custom journal style, feel free to delete these.

%% General page header settings.
\usepackage{fancyhdr}
\pagestyle{fancy}
\lhead{\footnotesize{\scshape Draft paper}, {\footnotesize nnn:i (pp), Year Month day}}
\rhead{\scshape\footnotesize YOUR-NAME et al.}
\cfoot{\thepage}
\setlength{\voffset}{0.75cm}
\setlength{\headsep}{0.2cm}
\setlength{\footskip}{0.75cm}
\renewcommand{\headrulewidth}{0pt}

%% Specific style for first page.
\fancypagestyle{firststyle}
{
  \lhead{\footnotesize{\scshape Draft paper}, nnn:i (pp), YYYY Month day\\
  \scriptsize \textcopyright YYYY, Your name. All rights reserved.}
  \rhead{\footnotesize \footnotesize \today, \currenttime\\}
}

%To set the style of the titles:
\usepackage{titlesec}
\titleformat{\section}
  {\centering\normalfont\uppercase}
  {\thesection.}
  {0em}
  { }
\titleformat{\subsection}
  {\centering\normalsize\slshape}
  {\thesubsection.}
  {0em}
  { }
\titleformat{\subsubsection}
  {\centering\small\slshape}
  {\thesubsubsection.}
  {0em}
  { }

%% Title and author information
\usepackage{authblk}
\renewcommand\Authfont{\small\scshape}
\renewcommand\Affilfont{\footnotesize\normalfont}
\setlength{\affilsep}{0.2cm}


==> tex/src/references.tex <==
%% Non-software BibTeX entries. The software-specific BibTeX entries are
%% stored in a '*.tex' file under the 'tex/dependencies' directory.
%
%% [[[BibTeX 0.99d complains with the at-character, even when its in a
%%    comment line! So ::at:: is used instead in the email address]]].
%% Copyright (C) 2018-2022 Mohammad Akhlaghi <mohammad::at::akhlaghi.org>
%% Copyright (C) 2022 Sepideh Eskandarlou <sepideh.eskandarlou::at::gmail.com>
%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{nunez23,
       author = {{Garate-Nu{\~n}ez}, Luc{\'\i}a P. and {Robotham}, Aaron S.~G. and {Bellstedt}, Sabine and {Davies}, Luke J.~M. and {Mart{\'\i}nez-Lombilla}, Cristina},
        title = "{The Hyper Suprime-Cam extended point spread functions and applications}",
      journal = {\mnras},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jun,
       volume = {531},
       number = {2},
        pages = {2517-2530},
          doi = {10.1093/mnras/stae1292},
archivePrefix = {arXiv},
       eprint = {2309.16244},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.531.2517G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{gaiadr3,
       author = {{Gaia Collaboration} and {Vallenari}, A. and {Brown}, A.~G.~A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Arenou}, F. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Ducourant}, C. and {Evans}, D.~W. and {Eyer}, L. and {Guerra}, R. and {Hutton}, A. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U.~L. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Tanga}, P. and {Walton}, N.~A. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Drimmel}, R. and {Jansen}, F. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Guerrier}, A. and {Heiter}, U. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P.~W. and {Busonero}, D. and {Busso}, G. and {C{\'a}novas}, H. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {de Teodoro}, P. and {Nu{\~n}ez Campos}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Esquej}, P. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fraile}, E. and {Garabato}, D. and {Garc{\'\i}a-Lario}, P. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Recio-Blanco}, A. and {Reyl{\'e}}, C. and {Riello}, M. and {Rimoldini}, L. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {Abbas}, U. and {{\'A}brah{\'a}m}, P. and {Abreu Aramburu}, A. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Aldea-Montero}, F. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anders}, F. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Binnenfeld}, A. and {Blanco-Cuaresma}, S. and {Blazere}, A. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiaramida}, V. and {Chiavassa}, A. and {Chornay}, N. and {Comoretto}, G. and {Contursi}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Cropper}, M. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R.},
        title = "{Gaia Data Release 3. Summary of the content and survey properties}",
      journal = {\aap},
     keywords = {techniques: photometric, techniques: spectroscopic, techniques: radial velocities, catalogs, astrometry, parallaxes, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jun,
       volume = {674},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202243940},
archivePrefix = {arXiv},
       eprint = {2208.00211},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...674A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{comeron18,
       author = {{Comer{\'o}n}, S. and {Salo}, H. and {Knapen}, J.~H.},
        title = "{The reports of thick discs' deaths are greatly exaggerated. Thick discs are NOT artefacts caused by diffuse scattered light}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: observational, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = feb,
       volume = {610},
          eid = {A5},
        pages = {A5},
          doi = {10.1051/0004-6361/201731415},
archivePrefix = {arXiv},
       eprint = {1709.00457},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...610A...5C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martinexlomnilla19,
       author = {{Mart{\'\i}nez-Lombilla}, C. and {Knapen}, J.~H.},
        title = "{Properties of extragalactic thick discs recovered from ultra-deep Stripe82 imaging}",
      journal = {\aap},
     keywords = {galaxies: formation, galaxies: evolution, galaxies: structure, methods: observational, methods: data analysis, techniques: image processing, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = sep,
       volume = {629},
          eid = {A12},
        pages = {A12},
          doi = {10.1051/0004-6361/201935464},
archivePrefix = {arXiv},
       eprint = {1907.02995},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...629A..12M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peters17,
       author = {{Peters}, S.~P.~C. and {van der Kruit}, P.~C. and {Knapen}, J.~H. and {Trujillo}, I. and {Fliri}, J. and {Cisternas}, M. and {Kelvin}, L.~S.},
        title = "{Stellar disc truncations and extended haloes in face-on spiral galaxies}",
      journal = {\mnras},
     keywords = {galaxies: photometry, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {427-444},
          doi = {10.1093/mnras/stx1205},
archivePrefix = {arXiv},
       eprint = {1705.03555},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470..427P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{knapen17,
       author = {{Knapen}, Johan H. and {Trujillo}, Ignacio},
        title = "{Ultra-Deep Imaging: Structure of Disks and Haloes}",
     keywords = {Physics, Astrophysics - Astrophysics of Galaxies},
    booktitle = {Outskirts of Galaxies},
         year = 2017,
       editor = {{Knapen}, Johan H. and {Lee}, Janice C. and {Gil de Paz}, Armando},
       series = {Astrophysics and Space Science Library},
       volume = {434},
        month = jan,
        pages = {255},
          doi = {10.1007/978-3-319-56570-5_8},
archivePrefix = {arXiv},
       eprint = {1612.05405},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ASSL..434..255K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Roychowdhury24,
       author = {{Roychowdhury}, Jyotika and {Derby}, Kevin and {Kim}, Daewook},
        title = "{Astronomical Image Processing Benchmark Study for Various Telescope Aperture Shapes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = feb,
          eid = {arXiv:2402.05233},
        pages = {arXiv:2402.05233},
          doi = {10.48550/arXiv.2402.05233},
archivePrefix = {arXiv},
       eprint = {2402.05233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240205233R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{Lanzetta23,
       author = {{Lanzetta}, Kenneth M. and {Gromoll}, Stefan and {Shara}, Michael M. and {Berg}, Stephen and {Garland}, James and {Mancini}, Evan and {Valls-Gabaud}, David and {Walter}, Frederick M. and {Webb}, John K.},
        title = "{Introducing the Condor array telescope II - deep imaging observations of the edge-on spiral galaxy NGC 5907 and the NGC 5866 Group: yet another view of the iconic stellar stream}",
      journal = {\mnras},
     keywords = {Galaxies, galaxies: dwarf, galaxies: groups: individual, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = mar,
       volume = {529},
       number = {1},
        pages = {197-211},
          doi = {10.1093/mnras/stad3806},
archivePrefix = {arXiv},
       eprint = {2309.17248},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.529..197L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}













@ARTICLE{Berman23,
       author = {{Berman}, Edward and {McCleary}, Jacqueline},
        title = "{ShOpt.jl: A Julia Package for Empirical Point Spread Function Characterization of JWST NIRCam Data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Mathematics - Numerical Analysis},
         year = 2023,
        month = sep,
          eid = {arXiv:2310.00071},
        pages = {arXiv:2310.00071},
          doi = {10.48550/arXiv.2310.00071},
archivePrefix = {arXiv},
       eprint = {2310.00071},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv231000071B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{carlinhos23,
       author = {{L{\'o}pez-Sanjuan}, C. and {V{\'a}zquez Rami{\'o}}, H. and {Xiao}, K. and {Yuan}, H. and {Carrasco}, J.~M. and {Varela}, J. and {Crist{\'o}bal-Hornillos}, D. and {Tremblay}, P. -E. and {Ederoclite}, A. and {Mar{\'\i}n-Franch}, A. and {Cenarro}, A.~J. and {Coelho}, P.~R.~T. and {Daflon}, S. and {del Pino}, A. and {Dom{\'\i}nguez S{\'a}nchez}, H. and {Fern{\'a}ndez-Ontiveros}, J.~A. and {Hern{\'a}n-Caballero}, A. and {Jim{\'e}nez-Esteban}, F.~M. and {Alcaniz}, J. and {Angulo}, R.~E. and {Dupke}, R.~A. and {Hern{\'a}ndez-Monteagudo}, C. and {Moles}, M. and {Sodr{\'e}}, L.},
        title = "{J-PLUS: Toward a homogeneous photometric calibration using Gaia BP/RP low-resolution spectra}",
      journal = {\aap},
     keywords = {methods: statistical, techniques: photometric, surveys, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = mar,
       volume = {683},
          eid = {A29},
        pages = {A29},
          doi = {10.1051/0004-6361/202346012},
archivePrefix = {arXiv},
       eprint = {2301.12395},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...683A..29L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{liu22,
       author = {{Liu}, Qing and {Abraham}, Roberto and {Gilhuly}, Colleen and {van Dokkum}, Pieter and {Martin}, Peter G. and {Li}, Jiaxuan and {Greco}, Johnny P. and {Lokhorst}, Deborah and {Chen}, Seery and {Danieli}, Shany and {Keim}, Michael A. and {Merritt}, Allison and {Miller}, Tim B. and {Pasha}, Imad and {Polzin}, Ava and {Shen}, Zili and {Zhang}, Jielai},
        title = "{A Method to Characterize the Wide-angle Point-Spread Function of Astronomical Images}",
      journal = {\apj},
     keywords = {611, 622, 940, 1858, 1965, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {925},
       number = {2},
          eid = {219},
        pages = {219},
          doi = {10.3847/1538-4357/ac32c6},
archivePrefix = {arXiv},
       eprint = {2110.11598},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...925..219L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{nardiello22,
       author = {{Nardiello}, D. and {Bedin}, L.~R. and {Burgasser}, A. and {Salaris}, M. and {Cassisi}, S. and {Griggio}, M. and {Scalco}, M.},
        title = "{Photometry and astrometry with JWST - I. NIRCam point spread functions and the first JWST colour-magnitude diagrams of a globular cluster}",
      journal = {\mnras},
     keywords = {techniques: image processing, techniques: photometric, stars: Population II, white dwarfs, globular clusters: individual: NGC 6341 (M 92), Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2022,
        month = nov,
       volume = {517},
       number = {1},
        pages = {484-497},
          doi = {10.1093/mnras/stac2659},
archivePrefix = {arXiv},
       eprint = {2209.06547},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.517..484N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{homeister22,
       author = {{Hofmeister}, Stefan Johann and {Hahn}, Michael and {Savin}, Daniel Wolf},
        title = "{Deriving instrumental point spread functions from partially occulted images}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics, Physics - Optics},
         year = 2022,
        month = jul,
          eid = {arXiv:2207.03487},
        pages = {arXiv:2207.03487},
archivePrefix = {arXiv},
       eprint = {2207.03487},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220703487H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{borlaff22,
       author = {{Borlaff}, A.~S. and {G{\'o}mez-Alvarez}, P. and {Altieri}, B. and {Marcum}, P.~M. and {Vavrek}, R. and {Laureijs}, R. and {Kohley}, R. and {Buitrago}, F. and {Cuillandre}, J. -C. and {Duc}, P. -A. and {Gaspar Venancio}, L.~M. and {Amara}, A. and {Andreon}, S. and {Auricchio}, N. and {Azzollini}, R. and {Baccigalupi}, C. and {Balaguera-Antol{\'\i}nez}, A. and {Baldi}, M. and {Bardelli}, S. and {Bender}, R. and {Biviano}, A. and {Bodendorf}, C. and {Bonino}, D. and {Bozzo}, E. and {Branchini}, E. and {Brescia}, M. and {Brinchmann}, J. and {Burigana}, C. and {Cabanac}, R. and {Camera}, S. and {Candini}, G.~P. and {Capobianco}, V. and {Cappi}, A. and {Carbone}, C. and {Carretero}, J. and {Carvalho}, C.~S. and {Casas}, S. and {Castander}, F.~J. and {Castellano}, M. and {Castignani}, G. and {Cavuoti}, S. and {Cimatti}, A. and {Cledassou}, R. and {Colodro-Conde}, C. and {Congedo}, G. and {Conselice}, C.~J. and {Conversi}, L. and {Copin}, Y. and {Corcione}, L. and {Coupon}, J. and {Courtois}, H.~M. and {Cropper}, M. and {Da Silva}, A. and {Degaudenzi}, H. and {Di Ferdinando}, D. and {Douspis}, M. and {Dubath}, F. and {Duncan}, C.~A.~J. and {Dupac}, X. and {Dusini}, S. and {Ealet}, A. and {Fabricius}, M. and {Farina}, M. and {Farrens}, S. and {Ferreira}, P.~G. and {Ferriol}, S. and {Finelli}, F. and {Flose-Reimberg}, P. and {Fosalba}, P. and {Frailis}, M. and {Franceschi}, E. and {Fumana}, M. and {Galeotta}, S. and {Ganga}, K. and {Garilli}, B. and {Gillis}, B. and {Giocoli}, C. and {Gozaliasl}, G. and {Graci{\'a}-Carpio}, J. and {Grazian}, A. and {Grupp}, F. and {Haugan}, S.~V.~H. and {Holmes}, W. and {Hormuth}, F. and {Jahnke}, K. and {Keihanen}, E. and {Kermiche}, S. and {Kiessling}, A. and {Kilbinger}, M. and {Kirkpatrick}, C.~C. and {Kitching}, T. and {Knapen}, J.~H. and {Kubik}, B. and {K{\"u}mmel}, M. and {Kunz}, M. and {Kurki-Suonio}, H. and {Liebing}, P. and {Ligori}, S. and {Lilje}, P.~B. and {Lindholm}, V. and {Lloro}, I. and {Mainetti}, G. and {Maino}, D. and {Mansutti}, O. and {Marggraf}, O. and {Markovic}, K. and {Martinelli}, M. and {Martinet}, N. and {Mart{\'\i}nez-Delgado}, D. and {Marulli}, F. and {Massey}, R. and {Maturi}, M. and {Maurogordato}, S. and {Medinaceli}, E. and {Mei}, S. and {Meneghetti}, M. and {Merlin}, E. and {Metcalf}, R.~B. and {Meylan}, G. and {Moresco}, M. and {Morgante}, G. and {Moscardini}, L. and {Munari}, E. and {Nakajima}, R. and {Neissner}, C. and {Niemi}, S.~M. and {Nightingale}, J.~W. and {Nucita}, A. and {Padilla}, C. and {Paltani}, S. and {Pasian}, F. and {Patrizii}, L. and {Pedersen}, K. and {Percival}, W.~J. and {Pettorino}, V. and {Pires}, S. and {Poncet}, M. and {Popa}, L. and {Potter}, D. and {Pozzetti}, L. and {Raison}, F. and {Rebolo}, R. and {Renzi}, A. and {Rhodes}, J. and {Riccio}, G. and {Romelli}, E. and {Roncarelli}, M. and {Rosset}, C. and {Rossetti}, E. and {Saglia}, R. and {S{\'a}nchez}, A.~G. and {Sapone}, D. and {Sauvage}, M. and {Schneider}, P. and {Scottez}, V. and {Secroun}, A. and {Seidel}, G. and {Serrano}, S. and {Sirignano}, C. and {Sirri}, G. and {Skottfelt}, J. and {Stanco}, L. and {Starck}, J.~L. and {Sureau}, F. and {Tallada-Cresp{\'\i}}, P. and {Taylor}, A.~N. and {Tenti}, M. and {Tereno}, I. and {Teyssier}, R. and {Toledo-Moreo}, R. and {Torradeflot}, F. and {Tutusaus}, I. and {Valentijn}, E.~A. and {Valenziano}, L. and {Valiviita}, J. and {Vassallo}, T. and {Viel}, M. and {Wang}, Y. and {Weller}, J. and {Whittaker}, L. and {Zacchei}, A. and {Zamorani}, G. and {Zucca}, E.},
        title = "{Euclid preparation. XVI. Exploring the ultra-low surface brightness Universe with Euclid/VIS}",
      journal = {\aap},
     keywords = {instrumentation: detectors, techniques: image processing, space vehicles: instruments, techniques: photometric, methods: observational, galaxies: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jan,
       volume = {657},
          eid = {A92},
        pages = {A92},
          doi = {10.1051/0004-6361/202141935},
archivePrefix = {arXiv},
       eprint = {2108.10321},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...657A..92E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{maneage,
       author = {{Akhlaghi}, Mohammad and {Infante-Sainz}, Raul and
         {Roukema}, Boudewijn F. and {Khellat}, Mohammadreza and
         {Valls-Gabaud}, David and {Baena-Galle}, Roberto},
        title = "{Toward Long-Term and Archivable Reproducibility}",
      journal = {CiSE},
     keywords = {Computer Science - Digital Libraries},
         year = 2021,
        month = may,
       volume = {23},
       number = {3},
        pages = {82-91},
          doi = {10.1109/MCSE.2021.3072860},
archivePrefix = {arXiv},
       eprint = {2006.03018},
 primaryClass = {cs.DL},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021CSE....23c..82A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{gillis20,
       author = {{Gillis}, Bryan R. and {Schrabback}, Tim and {Marggraf}, Ole and {Mandelbaum}, Rachel and {Massey}, Richard and {Rhodes}, Jason and {Taylor}, Andy},
        title = "{Validation of PSF models for HST and other space-based observations}",
      journal = {\mnras},
     keywords = {methods: data analysis, gravitational lensing: weak, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {4},
        pages = {5017-5038},
          doi = {10.1093/mnras/staa1818},
archivePrefix = {arXiv},
       eprint = {2006.14703},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.5017G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{infantesainz20,
       author = {{Infante-Sainz}, Ra{\'u}l and {Trujillo}, Ignacio and
         {Rom{\'a}n}, Javier},
        title = "{The Sloan Digital Sky Survey extended point spread functions}",
      journal = {MNRAS},
         year = 2020,
        month = feb,
       volume = {491},
       number = {4},
        pages = {5317-5329},
          doi = {10.1093/mnras/stz3111},
archivePrefix = {arXiv},
       eprint = {1911.01430},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5317I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{akhlaghi19,
       author = {{Akhlaghi}, Mohammad},
        title = "{Carving out the low surface brightness universe with NoiseChisel}",
      journal = {IAU Symposium 335},
         year = 2019,
        month = sep,
          eid = {arXiv:1909.11230},
        pages = {arXiv:1909.11230},
archivePrefix = {arXiv},
       eprint = {1909.11230},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190911230A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@INPROCEEDINGS{akhlaghi19b,
       author = {{Akhlaghi}, Mohammad},
        title = "{Separating Detection and Catalog Production}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Astronomical Data Analysis Software and Systems XXVI},
         year = 2019,
       editor = {{Molinaro}, Marco and {Shortridge}, Keith and {Pasian}, Fabio},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {521},
        month = oct,
        pages = {299},
          doi = {10.48550/arXiv.1611.06387},
archivePrefix = {arXiv},
       eprint = {1611.06387},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ASPC..521..299A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Eskandarlou24,
       author = {{Eskandarlou}, Sepideh and {Akhlaghi}, Mohammad},
        title = "{Gnuastro: Generating Polar Plots in Astronomical Images}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astronomy software, Open source software, Astronomical techniques, Spiral pitch angle, Spiral arms, 1855, 1866, 1684, 1561, 1559, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jun,
       volume = {8},
       number = {6},
          eid = {168},
        pages = {168},
          doi = {10.3847/2515-5172/ad5a6c},
archivePrefix = {arXiv},
       eprint = {2406.14619},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024RNAAS...8..168E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{nacho01a,
       author = {{Trujillo}, I. and {Aguerri}, J.~A.~L. and {Cepa}, J. and {Guti{\'e}rrez}, C.~M.},
        title = "{The effects of seeing on S{\`e}rsic profiles}",
      journal = {\mnras},
     keywords = {Astrophysics},
         year = 2001,
        month = feb,
       volume = {321},
       number = {2},
        pages = {269-276},
          doi = {10.1046/j.1365-8711.2001.03987.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0009097},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.321..269T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{nacho01b,
       author = {{Trujillo}, I. and {Aguerri}, J.~A.~L. and {Cepa}, J. and {Guti{\'e}rrez}, C.~M.},
        title = "{The effects of seeing on S{\'e}rsic profiles - II. The Moffat PSF}",
      journal = {\mnras},
     keywords = {ATMOSPHERIC EFFECTS, METHODS: DATA ANALYSIS, GALAXIES: DISTANCES AND REDSHIFTS, GALAXIES: PHOTOMETRY, Astrophysics},
         year = 2001,
        month = dec,
       volume = {328},
       number = {3},
        pages = {977-985},
          doi = {10.1046/j.1365-8711.2001.04937.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0109067},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.328..977T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{vandokkum19,
       author = {{van Dokkum}, Pieter and {Gilhuly}, Colleen and {Bonaca}, Ana and {Merritt}, Allison and {Danieli}, Shany and {Lokhorst}, Deborah and {Abraham}, Roberto and {Conroy}, Charlie and {Greco}, Johnny P.},
        title = "{Dragonfly Imaging of the Galaxy NGC 5907: A Different View of the Iconic Stellar Stream}",
      journal = {\apjl},
     keywords = {Tidal disruption, Dwarf galaxies, Low surface brightness galaxies, 1696, 416, 940, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {883},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.3847/2041-8213/ab40c9},
archivePrefix = {arXiv},
       eprint = {1906.11260},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...883L..32V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{minijpas,
       author = {{Bonoli}, S. and {Mar{\'\i}n-Franch}, A. and {Varela}, J. and {V{\'a}zquez Rami{\'o}}, H. and {Abramo}, L.~R. and {Cenarro}, A.~J. and {Dupke}, R.~A. and {V{\'\i}lchez}, J.~M. and {Crist{\'o}bal-Hornillos}, D. and {Gonz{\'a}lez Delgado}, R.~M. and {Hern{\'a}ndez-Monteagudo}, C. and {L{\'o}pez-Sanjuan}, C. and {Muniesa}, D.~J. and {Civera}, T. and {Ederoclite}, A. and {Hern{\'a}n-Caballero}, A. and {Marra}, V. and {Baqui}, P.~O. and {Cortesi}, A. and {Cypriano}, E.~S. and {Daflon}, S. and {de Amorim}, A.~L. and {D{\'\i}az-Garc{\'\i}a}, L.~A. and {Diego}, J.~M. and {Mart{\'\i}nez-Solaeche}, G. and {P{\'e}rez}, E. and {Placco}, V.~M. and {Prada}, F. and {Queiroz}, C. and {Alcaniz}, J. and {Alvarez-Candal}, A. and {Cepa}, J. and {Maroto}, A.~L. and {Roig}, F. and {Siffert}, B.~B. and {Taylor}, K. and {Benitez}, N. and {Moles}, M. and {Sodr{\'e}}, L. and {Carneiro}, S. and {Mendes de Oliveira}, C. and {Abdalla}, E. and {Angulo}, R.~E. and {Aparicio Resco}, M. and {Balaguera-Antol{\'\i}nez}, A. and {Ballesteros}, F.~J. and {Brito-Silva}, D. and {Broadhurst}, T. and {Carrasco}, E.~R. and {Castro}, T. and {Cid Fernandes}, R. and {Coelho}, P. and {de Melo}, R.~B. and {Doubrawa}, L. and {Fernandez-Soto}, A. and {Ferrari}, F. and {Finoguenov}, A. and {Garc{\'\i}a-Benito}, R. and {Iglesias-P{\'a}ramo}, J. and {Jim{\'e}nez-Teja}, Y. and {Kitaura}, F.~S. and {Laur}, J. and {Lopes}, P.~A.~A. and {Lucatelli}, G. and {Mart{\'\i}nez}, V.~J. and {Maturi}, M. and {Overzier}, R.~A. and {Pigozzo}, C. and {Quartin}, M. and {Rodr{\'\i}guez-Mart{\'\i}n}, J.~E. and {Salzano}, V. and {Tamm}, A. and {Tempel}, E. and {Umetsu}, K. and {Valdivielso}, L. and {von Marttens}, R. and {Zitrin}, A. and {D{\'\i}az-Mart{\'\i}n}, M.~C. and {L{\'o}pez-Alegre}, G. and {L{\'o}pez-Sainz}, A. and {Yanes-D{\'\i}az}, A. and {Rueda-Teruel}, F. and {Rueda-Teruel}, S. and {Abril Iba{\~n}ez}, J. and {L Ant{\'o}n Bravo}, J. and {Bello Ferrer}, R. and {Bielsa}, S. and {Casino}, J.~M. and {Castillo}, J. and {Chueca}, S. and {Cuesta}, L. and {Garzar{\'a}n Calderaro}, J. and {Iglesias-Marzoa}, R. and {{\'I}niguez}, C. and {Lamadrid Gutierrez}, J.~L. and {Lopez-Martinez}, F. and {Lozano-P{\'e}rez}, D. and {Ma{\'\i}cas Sacrist{\'a}n}, N. and {Molina-Ib{\'a}{\~n}ez}, E.~L. and {Moreno-Signes}, A. and {Rodr{\'\i}guez Llano}, S. and {Royo Navarro}, M. and {Tilve Rua}, V. and {Andrade}, U. and {Alfaro}, E.~J. and {Akras}, S. and {Arnalte-Mur}, P. and {Ascaso}, B. and {Barbosa}, C.~E. and {Beltr{\'a}n Jim{\'e}nez}, J. and {Benetti}, M. and {Bengaly}, C.~A.~P. and {Bernui}, A. and {Blanco-Pillado}, J.~J. and {Borges Fernandes}, M. and {Bregman}, J.~N. and {Bruzual}, G. and {Calderone}, G. and {Carvano}, J.~M. and {Casarini}, L. and {Chaves-Montero}, J. and {Chies-Santos}, A.~L. and {Coutinho de Carvalho}, G. and {Dimauro}, P. and {Duarte Puertas}, S. and {Figueruelo}, D. and {Gonz{\'a}lez-Serrano}, J.~I. and {Guerrero}, M.~A. and {Gurung-L{\'o}pez}, S. and {Herranz}, D. and {Huertas-Company}, M. and {Irwin}, J.~A. and {Izquierdo-Villalba}, D. and {Kanaan}, A. and {Kehrig}, C. and {Kirkpatrick}, C.~C. and {Lim}, J. and {Lopes}, A.~R. and {Lopes de Oliveira}, R. and {Marcos-Caballero}, A. and {Mart{\'\i}nez-Delgado}, D. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Mart{\'\i}nez-Somonte}, G. and {Oliveira}, N. and {Orsi}, A.~A. and {Penna-Lima}, M. and {Reis}, R.~R.~R. and {Spinoso}, D. and {Tsujikawa}, S. and {Vielva}, P. and {Vitorelli}, A.~Z. and {Xia}, J.~Q. and {Yuan}, H.~B. and {Arroyo-Polonio}, A. and {Dantas}, M.~L.~L. and {Galarza}, C.~A. and {Gon{\c{c}}alves}, D.~R. and {Gon{\c{c}}alves}, R.~S. and {Gonzalez}, J.~E. and {Gonzalez}, A.~H. and {Greisel}, N. and {Jim{\'e}nez-Esteban}, F. and {Landim}, R.~G. and {Lazzaro}, D. and {Magris}, G. and {Monteiro-Oliveira}, R. and {Pereira}, C.~B. and {Rebou{\c{c}}as}, M.~J. and {Rodriguez-Espinosa}, J.~M. and {Santos da Costa}, S. and {Telles}, E.},
        title = "{The miniJPAS survey: A preview of the Universe in 56 colors}",
      journal = {\aap},
     keywords = {surveys, techniques: photometric, astronomical databases: miscellaneous, stars: general, galaxies: general, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A31},
        pages = {A31},
          doi = {10.1051/0004-6361/202038841},
archivePrefix = {arXiv},
       eprint = {2007.01910},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{cenarro19,
       author = {{Cenarro}, A.~J. and {Moles}, M. and {Crist{\'o}bal-Hornillos}, D. and {Mar{\'\i}n-Franch}, A. and {Ederoclite}, A. and {Varela}, J. and {L{\'o}pez-Sanjuan}, C. and {Hern{\'a}ndez-Monteagudo}, C. and {Angulo}, R.~E. and {V{\'a}zquez Rami{\'o}}, H. and {Viironen}, K. and {Bonoli}, S. and {Orsi}, A.~A. and {Hurier}, G. and {San Roman}, I. and {Greisel}, N. and {Vilella-Rojo}, G. and {D{\'\i}az-Garc{\'\i}a}, L.~A. and {Logro{\~n}o-Garc{\'\i}a}, R. and {Gurung-L{\'o}pez}, S. and {Spinoso}, D. and {Izquierdo-Villalba}, D. and {Aguerri}, J.~A.~L. and {Allende Prieto}, C. and {Bonatto}, C. and {Carvano}, J.~M. and {Chies-Santos}, A.~L. and {Daflon}, S. and {Dupke}, R.~A. and {Falc{\'o}n-Barroso}, J. and {Gon{\c{c}}alves}, D.~R. and {Jim{\'e}nez-Teja}, Y. and {Molino}, A. and {Placco}, V.~M. and {Solano}, E. and {Whitten}, D.~D. and {Abril}, J. and {Ant{\'o}n}, J.~L. and {Bello}, R. and {Bielsa de Toledo}, S. and {Castillo-Ram{\'\i}rez}, J. and {Chueca}, S. and {Civera}, T. and {D{\'\i}az-Mart{\'\i}n}, M.~C. and {Dom{\'\i}nguez-Mart{\'\i}nez}, M. and {Garzar{\'a}n-Calderaro}, J. and {Hern{\'a}ndez-Fuertes}, J. and {Iglesias-Marzoa}, R. and {I{\~n}iguez}, C. and {Jim{\'e}nez Ruiz}, J.~M. and {Kruuse}, K. and {Lamadrid}, J.~L. and {Lasso-Cabrera}, N. and {L{\'o}pez-Alegre}, G. and {L{\'o}pez-Sainz}, A. and {Ma{\'\i}cas}, N. and {Moreno-Signes}, A. and {Muniesa}, D.~J. and {Rodr{\'\i}guez-Llano}, S. and {Rueda-Teruel}, F. and {Rueda-Teruel}, S. and {Soriano-Lagu{\'\i}a}, I. and {Tilve}, V. and {Valdivielso}, L. and {Yanes-D{\'\i}az}, A. and {Alcaniz}, J.~S. and {Mendes de Oliveira}, C. and {Sodr{\'e}}, L. and {Coelho}, P. and {Lopes de Oliveira}, R. and {Tamm}, A. and {Xavier}, H.~S. and {Abramo}, L.~R. and {Akras}, S. and {Alfaro}, E.~J. and {Alvarez-Candal}, A. and {Ascaso}, B. and {Beasley}, M.~A. and {Beers}, T.~C. and {Borges Fernandes}, M. and {Bruzual}, G.~R. and {Buzzo}, M.~L. and {Carrasco}, J.~M. and {Cepa}, J. and {Cortesi}, A. and {Costa-Duarte}, M.~V. and {De Pr{\'a}}, M. and {Favole}, G. and {Galarza}, A. and {Galbany}, L. and {Garcia}, K. and {Gonz{\'a}lez Delgado}, R.~M. and {Gonz{\'a}lez-Serrano}, J.~I. and {Guti{\'e}rrez-Soto}, L.~A. and {Hernandez-Jimenez}, J.~A. and {Kanaan}, A. and {Kuncarayakti}, H. and {Landim}, R.~C.~G. and {Laur}, J. and {Licandro}, J. and {Lima Neto}, G.~B. and {Lyman}, J.~D. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Miralda-Escud{\'e}}, J. and {Morate}, D. and {Nogueira-Cavalcante}, J.~P. and {Novais}, P.~M. and {Oncins}, M. and {Oteo}, I. and {Overzier}, R.~A. and {Pereira}, C.~B. and {Rebassa-Mansergas}, A. and {Reis}, R.~R.~R. and {Roig}, F. and {Sako}, M. and {Salvador-Rusi{\~n}ol}, N. and {Sampedro}, L. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Santos}, W.~A. and {Schmidtobreick}, L. and {Siffert}, B.~B. and {Telles}, E. and {Vilchez}, J.~M.},
        title = "{J-PLUS: The Javalambre Photometric Local Universe Survey}",
      journal = {\aap},
     keywords = {surveys, astronomical databases: miscellaneous, techniques: photometric, stars: general, Galaxy: general, galaxies: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A176},
        pages = {A176},
          doi = {10.1051/0004-6361/201833036},
archivePrefix = {arXiv},
       eprint = {1804.02667},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A.176C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{coupon18,
       author = {{Coupon}, Jean and {Czakon}, Nicole and {Bosch}, James and {Komiyama}, Yutaka and {Medezinski}, Elinor and {Miyazaki}, Satoshi and {Oguri}, Masamune},
        title = "{The bright-star masks for the HSC-SSP survey}",
      journal = {\pasj},
     keywords = {cosmology: observations, galaxies: photometry, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = jan,
       volume = {70},
          eid = {S7},
        pages = {S7},
          doi = {10.1093/pasj/psx047},
archivePrefix = {arXiv},
       eprint = {1705.00622},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PASJ...70S...7C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{xin18,
       author = {{Xin}, Bo and {Ivezi{\'c}}, {\v{Z}}eljko and {Lupton}, Robert H. and {Peterson}, John R. and {Yoachim}, Peter and {Jones}, R. Lynne and {Claver}, Charles F. and {Angeli}, George},
        title = "{A Study of the Point-spread Function in SDSS Images}",
      journal = {\aj},
     keywords = {atmospheric effects, instrumentation: detectors, methods: observational, stars: imaging, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = nov,
       volume = {156},
       number = {5},
          eid = {222},
        pages = {222},
          doi = {10.3847/1538-3881/aae316},
archivePrefix = {arXiv},
       eprint = {1805.02845},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..222X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{trujillo16,
       author = {{Trujillo}, Ignacio and {Fliri}, J{\"u}ergen},
        title = "{Beyond 31 mag arcsec$^{-2}$: The Frontier of Low Surface Brightness Imaging with the Largest Optical Telescopes}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: halos, galaxies: photometry, galaxies: spiral, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = jun,
       volume = {823},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/0004-637X/823/2/123},
archivePrefix = {arXiv},
       eprint = {1510.04696},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823..123T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{raul24,
         author = {{Infante-Sainz}, Ra{\'u}l and {Akhlaghi}, Mohammad and {Eskandarlou}, Sepideh},
          title = "{Gnuastro: Measuring Radial Profiles from Images}",
        journal = {Research Notes of the American Astronomical Society},
       keywords = {Astronomy software, Astronomical techniques, Astronomy data visualization, Broad band photometry, Open source software, 1855, 1684, 1968, 184, 1866},
           year = 2024,
          month = jan,
         volume = {8},
         number = {1},
            eid = {22},
          pages = {22},
            doi = {10.3847/2515-5172/ad1ee2},
  archivePrefix = {arXiv},
         eprint = {2401.05303},
   primaryClass = {astro-ph.IM},
         adsurl = {https://ui.adsabs.harvard.edu/abs/2024RNAAS...8...22I},
        adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@INPROCEEDINGS{Antonio15,
       author = {{Marin-Franch}, Antonio and {Taylor}, Keith and {Cenarro}, Javier and {Cristobal-Hornillos}, David and {Moles}, Mariano},
        title = "{T80Cam: a wide field camera for the J-PLUS survey}",
    booktitle = {IAU General Assembly},
         year = 2015,
       volume = {29},
        month = aug,
          eid = {2257381},
        pages = {2257381},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015IAUGA..2257381M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{jimenez15,
       author = {{Jim{\'e}nez-Teja}, Y. and {Ben{\'\i}tez}, N. and {Molino}, A. and {Fernandes}, C.~A.~C.},
        title = "{Accurate PSF-matched photometry and photometric redshifts for the extreme deep field with the Chebyshev-Fourier functions}",
      journal = {\mnras},
     keywords = {methods: data analysis, astronomical data bases: catalogues, techniques: photometric, galaxies: distances and redshifts, galaxies: photometry, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = oct,
       volume = {453},
       number = {1},
        pages = {1136-1146},
          doi = {10.1093/mnras/stv1612},
archivePrefix = {arXiv},
       eprint = {1507.04750},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.1136J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@INPROCEEDINGS{cenarro14,
       author = {{Cenarro}, A.~J. and {Moles}, M. and {Mar{\'\i}n-Franch}, A. and {Crist{\'o}bal-Hornillos}, D. and {Yanes D{\'\i}az}, A. and {Ederoclite}, A. and {Varela}, J. and {V{\'a}zquez Rami{\'o}}, H. and {Valdivielso}, L. and {Ben{\'\i}tez}, N. and {Cepa}, J. and {Dupke}, R. and {Fern{\'a}ndez-Soto}, A. and {Mendes de Oliveira}, C. and {Sodr{\'e}}, L. and {Taylor}, K. and {Rueda-Teruel}, S. and {Rueda-Teruel}, F. and {Luis-Simoes}, R. and {Chueca}, S. and {Ant{\'o}n}, J.~L. and {Bello}, R. and {D{\'\i}az-Mart{\'\i}n}, M.~C. and {Guill{\'e}n-Civera}, L. and {Hern{\'a}ndez-Fuertes}, J. and {Iglesias-Marzoa}, R. and {Jim{\'e}nez-Mej{\'\i}as}, D. and {Lasso-Cabrera}, N.~M. and {L{\'o}pez-Alegre}, G. and {L{\'o}pez-Sainz}, A. and {Rodr{\'\i}guez-Hern{\'a}ndez}, M.~A.~C. and {Su{\'a}rez}, O. and {Lamadrid}, J.~L. and {Ma{\'\i}cas}, N. and {Abril-Iba{\~n}ez}, J. and {Tilve}, V. and {Rodr{\'\i}guez-Llano}, S.},
        title = "{The Observatorio Astrof{\'\i}sico de Javalambre: current status, developments, operations, and strategies}",
    booktitle = {Observatory Operations: Strategies, Processes, and Systems V},
         year = 2014,
       editor = {{Peck}, Alison B. and {Benn}, Chris R. and {Seaman}, Robert L.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9149},
        month = aug,
          eid = {91491I},
        pages = {91491I},
          doi = {10.1117/12.2055455},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9149E..1IC},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{abraham14,
       author = {{Abraham}, Roberto G. and {van Dokkum}, Pieter G.},
        title = "{Ultra-Low Surface Brightness Imaging with the Dragonfly Telephoto Array}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jan,
       volume = {126},
       number = {935},
        pages = {55},
          doi = {10.1086/674875},
archivePrefix = {arXiv},
       eprint = {1401.5473},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PASP..126...55A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{slater09,
       author = {{Slater}, Colin T. and {Harding}, Paul and {Mihos}, J. Christopher},
        title = "{Removing Internal Reflections from Deep Imaging Data Sets}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2009,
        month = nov,
       volume = {121},
       number = {885},
        pages = {1267},
          doi = {10.1086/648457},
archivePrefix = {arXiv},
       eprint = {0909.3320},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009PASP..121.1267S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{martinz08,
       author = {{Mart{\'\i}nez-Delgado}, David and {Pe{\~n}arrubia}, Jorge and {Gabany}, R. Jay and {Trujillo}, Ignacio and {Majewski}, Steven R. and {Pohlen}, M.},
        title = "{The Ghost of a Dwarf Galaxy: Fossils of the Hierarchical Formation of the Nearby Spiral Galaxy NGC 5907}",
      journal = {\apj},
     keywords = {dark matter, galaxies: dwarf, galaxies: evolution, galaxies: halos, galaxies: individual: NGC 5907, galaxies: interactions, Astrophysics},
         year = 2008,
        month = dec,
       volume = {689},
       number = {1},
        pages = {184-193},
          doi = {10.1086/592555},
archivePrefix = {arXiv},
       eprint = {0805.1137},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...689..184M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{mighell05,
       author = {{Mighell}, Kenneth J.},
        title = "{Stellar photometry and astrometry with discrete point spread functions}",
      journal = {\mnras},
     keywords = {methods: analytical, methods: numerical, methods: statistical, techniques: image processing, techniques photometric, astrometry, Astrophysics},
         year = 2005,
        month = aug,
       volume = {361},
       number = {3},
        pages = {861-878},
          doi = {10.1111/j.1365-2966.2005.09208.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0505455},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.361..861M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{idiart02,
       author = {{Idiart}, T.~P. and {Michard}, R. and {de Freitas Pacheco}, J.~A.},
        title = "{New UBVRI colour distributions in E-type galaxies . I. The data}",
      journal = {\aap},
     keywords = {GALAXIES: ELLIPTICAL AND LENTICULARS, CD, GALAXIES: ISM},
         year = 2002,
        month = jan,
       volume = {383},
        pages = {30-45},
          doi = {10.1051/0004-6361:20011699},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...383...30I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{michard02,
       author = {{Michard}, R.},
        title = "{PSF far wings and ``red halo'' in the photometry of galaxies. One more source of errors}",
      journal = {\aap},
     keywords = {GALAXIES: ELLIPTICAL AND LENTICULARS, CD, GALAXIES: PHOTOMETRY},
         year = 2002,
        month = mar,
       volume = {384},
        pages = {763-771},
          doi = {10.1051/0004-6361:20011813},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...384..763M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{anderson00,
       author = {{Anderson}, Jay and {King}, Ivan R.},
        title = "{Toward High-Precision Astrometry with WFPC2. I. Deriving an Accurate Point-Spread Function}",
      journal = {\pasp},
     keywords = {Astrometry, Methods: Data Analysis, Techniques: Image Processing, Techniques: Photometric, Astrophysics},
         year = 2000,
        month = oct,
       volume = {112},
       number = {776},
        pages = {1360-1382},
          doi = {10.1086/316632},
archivePrefix = {arXiv},
       eprint = {astro-ph/0006325},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000PASP..112.1360A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{hasan95,
       author = {{Hasan}, Hashima and {Burrows}, C.~J.},
        title = "{Telescope Image Modelling (TIM)}",
      journal = {\pasp},
     keywords = {Computer Programs, Computerized Simulation, Hubble Space Telescope, Images, Utilization, Autocorrelation, Data Sampling, Optical Equipment, Pixels, Point Spread Functions, Astronomy, METHODS: OBSERVATIONAL, TECHNIQUES: MISCELLANEOUS},
         year = 1995,
        month = mar,
       volume = {107},
        pages = {289},
          doi = {10.1086/133552},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995PASP..107..289H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{middlemass89,
       author = {{Middlemass}, D. and {Clegg}, R.~E.~S. and {Walsh}, J.~R.},
        title = "{The giant haloes of NGC 6543 and 6826.}",
      journal = {\mnras},
     keywords = {Giant Stars, Halos, Planetary Nebulae, Stellar Envelopes, Stellar Spectra, Astronomical Spectroscopy, Forbidden Transitions, Oxygen Spectra, Spectrum Analysis, Stellar Winds, Astrophysics},
         year = 1989,
        month = jul,
       volume = {239},
        pages = {1-17},
          doi = {10.1093/mnras/239.1.1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989MNRAS.239....1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{king71,
       author = {{King}, Ivan R.},
        title = "{The Profile of a Star Image}",
      journal = {\pasp},
         year = 1971,
        month = apr,
       volume = {83},
       number = {492},
        pages = {199},
          doi = {10.1086/129100},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971PASP...83..199K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{moffat69,
       author = {{Moffat}, A.~F.~J.},
        title = "{A Theoretical Investigation of Focal Stellar Images in the Photographic Emulsion and Application to Photographic Photometry}",
      journal = {\aap},
         year = 1969,
        month = dec,
       volume = {3},
        pages = {455},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969A&A.....3..455M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{devacouleurs58,
       author = {{de Vaucouleurs}, G.},
        title = "{Photoelectric photometry of the Andromeda Nebula in the UBV system.}",
      journal = {\apj},
         year = 1958,
        month = nov,
       volume = {128},
        pages = {465},
          doi = {10.1086/146564},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958ApJ...128..465D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{gaia16,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland}, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{gaia23,
       author = {{Gaia Collaboration} and {Vallenari}, A. and {Brown}, A.~G.~A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Arenou}, F. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Ducourant}, C. and {Evans}, D.~W. and {Eyer}, L. and {Guerra}, R. and {Hutton}, A. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U.~L. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Tanga}, P. and {Walton}, N.~A. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Drimmel}, R. and {Jansen}, F. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Guerrier}, A. and {Heiter}, U. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P.~W. and {Busonero}, D. and {Busso}, G. and {C{\'a}novas}, H. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {de Teodoro}, P. and {Nu{\~n}ez Campos}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Esquej}, P. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fraile}, E. and {Garabato}, D. and {Garc{\'\i}a-Lario}, P. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Recio-Blanco}, A. and {Reyl{\'e}}, C. and {Riello}, M. and {Rimoldini}, L. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {Abbas}, U. and {{\'A}brah{\'a}m}, P. and {Abreu Aramburu}, A. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Aldea-Montero}, F. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anders}, F. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Binnenfeld}, A. and {Blanco-Cuaresma}, S. and {Blazere}, A. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiaramida}, V. and {Chiavassa}, A. and {Chornay}, N. and {Comoretto}, G. and {Contursi}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Cropper}, M. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delisle}, J. -B. and {Demouchy}, C. and {Dharmawardena}, T.~E. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Edvardsson}, B. and {Enke}, H. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fournier}, Y. and {Fouron}, C. and {Fragkoudi}, F. and {Gai}, M. and {Garcia-Gutierrez}, A. and {Garcia-Reinaldos}, M. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavel}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Santamar{\'\i}a}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guillout}, P. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Helmer}, A. and {Helmi}, A. and {Sarmiento}, M.~H. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jardine}, K. and {Jasniewicz}, G. and {Jean-Antoine Piccolo}, A. and {Jim{\'e}nez-Arranz}, {\'O}. and {Jorissen}, A. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {K{\'o}sp{\'a}l}, {\'A}. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Kun}, M. and {Laizeau}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E.~L. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Lorca}, A. and {Loup}, C. and {Madrero Pardo}, P. and {Magdaleno Romeo}, A. and {Managau}, S. and {Mann}, R.~G. and {Manteiga}, M. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos}, J. and {Marcos Santos}, M.~M.~S. and {Mar{\'\i}n Pina}, D. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Marton}, G. and {Mary}, N. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Monari}, G. and {Mongui{\'o}}, M. and {Montegriffo}, P. and {Montero}, A. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Nagy}, Z. and {Noval}, L. and {Oca{\~n}a}, F. and {Ogden}, A. and {Ordenovic}, C. and {Osinde}, J.~O. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Pallas-Quintela}, L. and {Panahi}, A. and {Payne-Wardenaar}, S. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Richards}, P.~J. and {Rios Diaz}, C. and {Ripepi}, V. and {Riva}, A. and {Rix}, H. -W. and {Rixon}, G. and {Robichon}, N. and {Robin}, A.~C. and {Robin}, C. and {Roelens}, M. and {Rogues}, H.~R.~O. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruz Mieres}, D. and {Rybicki}, K.~A. and {Sadowski}, G. and {S{\'a}ez N{\'u}{\~n}ez}, A. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Silvelo}, A. and {Slezak}, E. and {Slezak}, I. and {Smart}, R.~L. and {Snaith}, O.~N. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spina}, L. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Taylor}, M.~B. and {Teixeira}, R. and {Tolomei}, L. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Torralba Elipe}, G. and {Trabucchi}, M. and {Tsounis}, A.~T. and {Turon}, C. and {Ulla}, A. and {Unger}, N. and {Vaillant}, M.~V. and {van Dillen}, E. and {van Reeven}, W. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zwitter}, T.},
        title = "{Gaia Data Release 3. Summary of the content and survey properties}",
      journal = {\aap},
     keywords = {techniques: photometric, techniques: spectroscopic, techniques: radial velocities, catalogs, astrometry, parallaxes, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jun,
       volume = {674},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202243940},
archivePrefix = {arXiv},
       eprint = {2208.00211},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...674A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sandin14,
       author = {{Sandin}, Christer},
        title = "{The influence of diffuse scattered light. I. The PSF and its role in observations of the edge-on galaxy NGC 5907}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: observational, galaxies: structure, galaxies: individual: NGC 5907, telescopes, galaxies: halos, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = jul,
       volume = {567},
          eid = {A97},
        pages = {A97},
          doi = {10.1051/0004-6361/201423429},
archivePrefix = {arXiv},
       eprint = {1406.5508},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...567A..97S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sandin15,
       author = {{Sandin}, Christer},
        title = "{The influence of diffuse scattered light. II. Observations of galaxy haloes and thick discs and hosts of blue compact galaxies}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: observational, galaxies: fundamental, parameters, galaxies: halos, galaxies: structure, galaxies:, photometry, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = may,
       volume = {577},
          eid = {A106},
        pages = {A106},
          doi = {10.1051/0004-6361/201425168},
archivePrefix = {arXiv},
       eprint = {1502.07244},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...577A.106S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{roman20,
       author = {{Rom{\'a}n}, Javier and {Trujillo}, Ignacio and {Montes}, Mireia},
        title = "{Galactic cirri in deep optical imaging}",
      journal = {\aap},
     keywords = {ISM: clouds, dust, extinction, techniques: image processing, techniques: photometric, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {644},
          eid = {A42},
        pages = {A42},
          doi = {10.1051/0004-6361/201936111},
archivePrefix = {arXiv},
       eprint = {1907.00978},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...644A..42R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{mihos13,
       author = {{Mihos}, J. Christopher and {Harding}, Paul and {Spengler}, Chelsea E. and {Rudick}, Craig S. and {Feldmeier}, John J.},
        title = "{The Extended Optical Disk of M101}",
      journal = {\apj},
     keywords = {galaxies: individual: M101, galaxies: interactions, galaxies: spiral, galaxies: star formation, galaxies: stellar content, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = jan,
       volume = {762},
       number = {2},
          eid = {82},
        pages = {82},
          doi = {10.1088/0004-637X/762/2/82},
archivePrefix = {arXiv},
       eprint = {1211.3095},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...762...82M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{benitez14,
       author = {{Benitez}, N. and {Dupke}, R. and {Moles}, M. and {Sodre}, L. and {Cenarro}, J. and {Marin-Franch}, A. and {Taylor}, K. and {Cristobal}, D. and {Fernandez-Soto}, A. and {Mendes de Oliveira}, C. and {Cepa-Nogue}, J. and {Abramo}, L.~R. and {Alcaniz}, J.~S. and {Overzier}, R. and {Hernandez-Monteagudo}, C. and {Alfaro}, E.~J. and {Kanaan}, A. and {Carvano}, J.~M. and {Reis}, R.~R.~R. and {Martinez Gonzalez}, E. and {Ascaso}, B. and {Ballesteros}, F. and {Xavier}, H.~S. and {Varela}, J. and {Ederoclite}, A. and {Vazquez Ramio}, H. and {Broadhurst}, T. and {Cypriano}, E. and {Angulo}, R. and {Diego}, J.~M. and {Zandivarez}, A. and {Diaz}, E. and {Melchior}, P. and {Umetsu}, K. and {Spinelli}, P.~F. and {Zitrin}, A. and {Coe}, D. and {Yepes}, G. and {Vielva}, P. and {Sahni}, V. and {Marcos-Caballero}, A. and {Kitaura}, F. -S. and {Maroto}, A.~L. and {Masip}, M. and {Tsujikawa}, S. and {Carneiro}, S. and {Gonzalez Nuevo}, J. and {Carvalho}, G.~C. and {Reboucas}, M.~J. and {Carvalho}, J.~C. and {Abdalla}, E. and {Bernui}, A. and {Pigozzo}, C. and {Ferreira}, E.~G.~M. and {Chandrachani Devi}, N. and {Bengaly}, C.~A.~P., Jr. and {Campista}, M. and {Amorim}, A. and {Asari}, N.~V. and {Bongiovanni}, A. and {Bonoli}, S. and {Bruzual}, G. and {Cardiel}, N. and {Cava}, A. and {Cid Fernandes}, R. and {Coelho}, P. and {Cortesi}, A. and {Delgado}, R.~G. and {Diaz Garcia}, L. and {Espinosa}, J.~M.~R. and {Galliano}, E. and {Gonzalez-Serrano}, J.~I. and {Falcon-Barroso}, J. and {Fritz}, J. and {Fernandes}, C. and {Gorgas}, J. and {Hoyos}, C. and {Jimenez-Teja}, Y. and {Lopez-Aguerri}, J.~A. and {Lopez-San Juan}, C. and {Mateus}, A. and {Molino}, A. and {Novais}, P. and {OMill}, A. and {Oteo}, I. and {Perez-Gonzalez}, P.~G. and {Poggianti}, B. and {Proctor}, R. and {Ricciardelli}, E. and {Sanchez-Blazquez}, P. and {Storchi-Bergmann}, T. and {Telles}, E. and {Schoennell}, W. and {Trujillo}, N. and {Vazdekis}, A. and {Viironen}, K. and {Daflon}, S. and {Aparicio-Villegas}, T. and {Rocha}, D. and {Ribeiro}, T. and {Borges}, M. and {Martins}, S.~L. and {Marcolino}, W. and {Martinez-Delgado}, D. and {Perez-Torres}, M.~A. and {Siffert}, B.~B. and {Calvao}, M.~O. and {Sako}, M. and {Kessler}, R. and {Alvarez-Candal}, A. and {De Pra}, M. and {Roig}, F. and {Lazzaro}, D. and {Gorosabel}, J. and {Lopes de Oliveira}, R. and {Lima-Neto}, G.~B. and {Irwin}, J. and {Liu}, J.~F. and {Alvarez}, E. and {Balmes}, I. and {Chueca}, S. and {Costa-Duarte}, M.~V. and {da Costa}, A.~A. and {Dantas}, M.~L.~L. and {Diaz}, A.~Y. and {Fabregat}, J. and {Ferrari}, F. and {Gavela}, B. and {Gracia}, S.~G. and {Gruel}, N. and {Gutierrez}, J.~L.~L. and {Guzman}, R. and {Hernandez-Fernandez}, J.~D. and {Herranz}, D. and {Hurtado-Gil}, L. and {Jablonsky}, F. and {Laporte}, R. and {Le Tiran}, L.~L. and {Licandro}, J and {Lima}, M. and {Martin}, E. and {Martinez}, V. and {Montero}, J.~J.~C. and {Penteado}, P. and {Pereira}, C.~B. and {Peris}, V. and {Quilis}, V. and {Sanchez-Portal}, M. and {Soja}, A.~C. and {Solano}, E. and {Torra}, J. and {Valdivielso}, L.},
        title = "{J-PAS: The Javalambre-Physics of the Accelerated Universe Astrophysical Survey}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = mar,
          eid = {arXiv:1403.5237},
        pages = {arXiv:1403.5237},
          doi = {10.48550/arXiv.1403.5237},
archivePrefix = {arXiv},
       eprint = {1403.5237},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1403.5237B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@INPROCEEDINGS{upad,
author = {{Crist{\'o}bal-Hornillos}, D. and {Gruel}, N. and {Varela}, J. and
{L{\'o}pez-Sainz}, A. and {Ederoclite}, A. and {Moles}, M. and
{Cenarro}, A.~J. and {Mar{\'{\i}}n-Franch}, A. and {Hern{\'a}ndez-Fuertes}, J. and
{Yanes-D{\'{\i}}az}, A. and {Chueca}, S. and {Rueda-Teruel}, S. and
{Rueda-Teruel}, F. and {Luis-Simoes}, R.},
title = "{J-PAS data management pipeline and archiving}",
booktitle = {SPIE CS},
year = 2012,
series = {},
volume = 8451,
month = sep,
eid = {845116},
doi = {10.1117/12.925431},
adsurl = {http://esoads.eso.org/abs/2012SPIE.8451E..16C},
adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@BOOK{gnuastrobook,
     author = {{Akhlaghi}, Mohammad},
      title = {GNU Astronomy Utilities (version 0.23), https://doi.org/10.5281/zenodo.12738457},
       year = 2024,
  publisher = {Free Software Foundation},
        doi = {10.5281/zenodo.12738457}
}








@INPROCEEDINGS{amir24,
       author = {{Bazkiaei}, Amir E. and {Kelvin}, Lee S. and {Brough}, Sarah and {O'Toole}, Simon J. and {Watkins}, Aaron and {Schmitz}, Morgan A.},
        title = "{Bright star subtraction pipeline for LSST: phase one report}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
    booktitle = {Software and Cyberinfrastructure for Astronomy VIII},
         year = 2024,
       editor = {{Ibsen}, Jorge and {Chiozzi}, Gianluca},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {13101},
        month = jul,
          eid = {131013N},
        pages = {131013N},
          doi = {10.1117/12.3019590},
archivePrefix = {arXiv},
       eprint = {2408.04387},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024SPIE13101E..3NB},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{nafise25,
       author = {{Sedighi}, Nafise and {Sharbaf}, Zahra and {Trujillo}, Ignacio and {Eskandarlou}, Sepideh and {Golini}, Giulia and {Infante-Sainz}, Ra{\'u}l and {Raji}, Samane and {Zaritsky}, Dennis and {Ardakani}, Pedram Ashofteh and {Chamba}, Nushkia and {Hosseini-ShahiSavandi}, S. Zahra and {Donnerstein}, Richard and {D'Onofrio}, Mauro and {Martin}, Garreth and {Montes}, Mireia and {Rom{\'a}n}, Javier},
        title = "{LIGHTS. The extended point spread functions of the LIGHTS survey at the LBT}",
      journal = {The Open Journal of Astrophysics},
     keywords = {Astrophysics of Galaxies},
         year = 2025,
        month = jun,
       volume = {8},
          eid = {73},
        pages = {73},
          doi = {10.33232/001c.140865},
archivePrefix = {arXiv},
       eprint = {2410.20190},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025OJAp....8E..73S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{liu23,
       author = {{Liu}, Qing and {Abraham}, Roberto and {Martin}, Peter G. and {Bowman}, William P. and {van Dokkum}, Pieter and {Janssens}, Steven R. and {Chen}, Seery and {Keim}, Michael A. and {Lokhorst}, Deborah and {Pasha}, Imad and {Shen}, Zili and {Zhang}, Jielai},
        title = "{A Recipe for Unbiased Background Modeling in Deep Wide-field Astronomical Images}",
      journal = {\apj},
     keywords = {Low surface brightness galaxies, Astronomy data reduction, Interstellar dust, Astronomy image processing, Astronomical techniques, Sky surveys, Diffuse nebulae, 940, 1861, 836, 2306, 1684, 1464, 382, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = aug,
       volume = {953},
       number = {1},
          eid = {7},
        pages = {7},
          doi = {10.3847/1538-4357/acdee3},
archivePrefix = {arXiv},
       eprint = {2306.07922},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...953....7L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{watkins24,
       author = {{Watkins}, Aaron E. and {Kaviraj}, Sugata and {Collins}, Chris C. and {Knapen}, Johan H. and {Kelvin}, Lee S. and {Duc}, Pierre-Alain and {Rom{\'a}n}, Javier and {Mihos}, J. Christopher},
        title = "{Strategies for optimal sky subtraction in the low surface brightness regime}",
      journal = {\mnras},
     keywords = {methods: observational, techniques: image processing, surveys, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = mar,
       volume = {528},
       number = {3},
        pages = {4289-4306},
          doi = {10.1093/mnras/stae236},
archivePrefix = {arXiv},
       eprint = {2401.12297},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.528.4289W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{li25,
       author = {{Liu}, Qing and {Abraham}, Roberto and {Martin}, Peter G. and {Bowman}, William P. and {Dokkum}, Pieter van and {Danieli}, Shany and {Patel}, Ekta and {Janssens}, Steven R. and {Shen}, Zili and {Chen}, Seery and {Karunakaran}, Ananthan and {Keim}, Michael A. and {Lokhorst}, Deborah and {Pasha}, Imad and {Welch}, Douglas L.},
        title = "{Fuzzy Galaxies or Cirrus? Decomposition of Galactic Cirrus in Deep Wide-field Images}",
      journal = {\apj},
     keywords = {Astronomy data reduction, Astronomy image processing, Interstellar dust, Low surface brightness galaxies, Sky surveys, 1861, 2306, 836, 940, 1464, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2025,
        month = feb,
       volume = {979},
       number = {2},
          eid = {175},
        pages = {175},
          doi = {10.3847/1538-4357/ad9b25},
archivePrefix = {arXiv},
       eprint = {2412.00933},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025ApJ...979..175L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {\aaps},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{dejong08,
       author = {{de Jong}, Roelof S.},
        title = "{Point spread function tails and the measurements of diffuse stellar halo light around edge-on disc galaxies}",
      journal = {\mnras},
     keywords = {methods: data analysis, galaxies: fundamental parameters, galaxies: haloes, galaxies: spiral, galaxies: structure, Astrophysics},
         year = 2008,
        month = aug,
       volume = {388},
       number = {4},
        pages = {1521-1527},
          doi = {10.1111/j.1365-2966.2008.13505.x},
archivePrefix = {arXiv},
       eprint = {0807.0229},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.388.1521D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

